Do Design Metrics Capture Developers Perception of Quality? An Empirical Study on Self-Affirmed Refactoring Activities

Background. Refactoring is a critical task in software maintenance and is generally performed to enforce the best design and implementation practices or to cope with design defects. Several studies attempted to detect refactoring activities through mining software repositories allowing to collect, analyze and get actionable data-driven insights about refactoring practices within software projects. Aim. We aim at identifying, among the various quality models presented in the literature, the ones that are more in-line with the developer's vision of quality optimization, when they explicitly mention that they are refactoring to improve them. Method. We extract a large corpus of design-related refactoring activities that are applied and documented by developers during their daily changes from 3,795 curated open source Java projects. In particular, we extract a large-scale corpus of structural metrics and anti-pattern enhancement changes, from which we identify 1,245 quality improvement commits with their corresponding refactoring operations, as perceived by software engineers. Thereafter, we empirically analyze the impact of these refactoring operations on a set of common state-of-the-art design quality metrics. Results. The statistical analysis of the obtained results shows that (i) a few state-of-the-art metrics are more popular than others; and (ii) some metrics are being more emphasized than others. Conclusions. We verify that there are a variety of structural metrics that can represent the internal quality attributes with different degrees of improvement and degradation of software quality. Most of the metrics that are mapped to the main quality attributes do capture developer intentions of quality improvement reported in the commit messages.

==> Charts/Approach.tex <==

\begin{figure}[h]
\centering
\begin{adjustbox}{width=0.5\textwidth}
\begin{tikzpicture}[node distance=2cm]

\node (start) [startstop] {Start};
\node (io) [io, right of=start, xshift=2cm] {Open Source Java projects};
\node (pro1) [process, right of=io,xshift=2cm] {Clone repositories};
\node (pro2) [process, below of=pro1, yshift=-0.1cm] {Detect refactorings};
\node (db1) [database, left of=pro2,xshift=-2cm,label=below:Refactoring commits log] {};
\node (pro3) [process, left of=db1, xshift=-2cm] {Extract commit messages};
\node (pro4) [process, below of=pro3, yshift=-0.1cm] {Select Quality Attributes};
\node (pro5) [process, right of=pro4, xshift=2cm] {Classify Commits};
\node (pro6) [process, right of=pro5, xshift=2cm] {Measure Quality Attributes};
\node (pro7) [process, below of=pro6, yshift=-0.1cm] {Compare Metrics Values};
\node (pro8) [process, left of =pro7, xshift=-2cm] {Identify Refactoring Sequences};
%\node (io2) [io, right of=pro4, xshift=2cm] {Refactoring patterns};
\node (stop) [startstop, left of =pro8, xshift=-2cm] {Stop};

\draw [arrow] (start) -- (io);
\draw [arrow] (io) -- (pro1);
\draw [arrow] (pro1) -- (pro2);
\draw [arrow] (pro2) -- (db1);
\draw [arrow] (db1) -- (pro3); 
\draw [arrow] (pro3) -- (pro4);
\draw [arrow] (pro4) -- (pro5);
\draw [arrow] (pro5) -- (pro6);
\draw [arrow] (pro6) -- (pro7);
\draw [arrow] (pro7) -- (pro8);
\draw [arrow] (pro8) -- (stop);

\end{tikzpicture}
\end{adjustbox}
\caption{Approach Overview.} 
\label{Chart:Approach Overview}
\end{figure}


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Sections/z-backup.tex <==

\begin{minipage}[t]{1\linewidth}
    \begin{itemize}
     \item{A variety of structural metrics can represent the internal quality attributes considered in this study. Based on our empirical investigation, for metrics that are associated with quality attributes, there are different degrees of improvement and degradation of software quality.}
    %\item Most of the metrics that are mapped to the main quality attributes, \textit{i.e.,} cohesion, coupling, and complexity, do capture developer intentions of quality improvement reported in the commit messages. In contrast, there is also a case in which the metrics do not capture quality improvement as perceived by developers. We summarize our findings as follows:}
      \item{Most of the metrics that are mapped to the main quality attributes, \textit{i.e.,} cohesion, coupling, and complexity, do capture developer intentions of quality improvement reported in the commit messages. In contrast, there is also a case in which the metrics do not capture quality improvement as perceived by developers. We summarize our findings as follows:}
      \begin{itemize}
        \item{\textbf{Cohesion.} In contrast with previous studies, cohesion tends to be well represented by LCOM as we found the metrics to be significantly improved in the refactored code (p-value $\leq$ 0.05).}
        \item{\textbf{Coupling.} Similarly to cohesion, optimizing the coupling quality attribute was empirically measured using both CBO and FANOUT (p-value $\leq$ 0.05), in comparison with FANIN and RFC.}
        \item{\textbf{Complexity.} One of the popular quality attributes that is being approximated by developers using a variety of metrics, namely CC, WMC, RFC, Evg, NPATH, and MaxNest (p-value $\leq$ 0.05).}
        \item{\textbf{Inheritance.} While DIT has been found be the metric that matches the developer's perception (p-value $\leq$ 0.05), NOC, known to be a measure for Inheritance in literature, tends to increase instead in practice (p-value $\leq$ 0.05).}
        \item{As for \textbf{Encapsulation}, \textbf{Abstraction} and \textbf{Design Size}. We cannot find any metric that can represent developer's intention of optimizing these quality attributes, and so these findings motivates a deeper investigation on understanding the mismatch between theory and practice.}
      \end{itemize}
    \end{itemize}
\end{minipage}

==> Tables/BoxPlotStatistics.tex <==
\begin{table*}[!htbp]
\begin{center}
\caption{Box Plot Statistics.}
\Eman{added this table to just help us with the discussion} \ali{to improve readability and if time permits, I suggest to color the columns background of each quality attribute with a different gray level color (since the are no vertical lines in the table, it is hard to delimit each quality attribute related columns; for example coupling columns in gray; coupling columns in white, complexity columns in gray, etc.)}
\label{Table:Box Plot Statistics.}
%\begin{sideways}
\begin{adjustbox}{width=1.15\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lllllllllllllllllllllllllllllllllllllllllllllllllllllll}
\toprule
\multirow{3}{*}{}      & \multicolumn{2}{c}{\textbf{Cohesion}}                  & \multicolumn{8}{c}{\textbf{Coupling}}                                                                                                             & \multicolumn{14}{c}{\textbf{Complexity}}                                                                                                  & \multicolumn{6}{c}{\textbf{Inheritance}}                                                                                                                                        \\
                    \cmidrule{2-32}
                       & \multicolumn{2}{c}{\textbf{LCOM}}                      & \multicolumn{2}{c}{\textbf{CBO}}                       & \multicolumn{2}{c}{\textbf{RFC}}                       & \multicolumn{2}{c}{\textbf{FANIN}}                     & \multicolumn{2}{c}{\textbf{FANOUT}}                    & \multicolumn{2}{c}{\textbf{CC}}                        & \multicolumn{2}{c}{\textbf{WMC}}                       & \multicolumn{2}{c}{\textbf{RFC}}                       & \multicolumn{2}{c}{\textbf{LCOM}}                      & \multicolumn{2}{c}{\textbf{Evg}} & %\multicolumn{1}{c}{\textbf{Evg}} &
                       \multicolumn{2}{c}{\textbf{NPATH}}                     & \multicolumn{2}{c}{\textbf{MaxNest}}                   & \multicolumn{2}{c}{\textbf{DIT}}                       & \multicolumn{2}{c}{\textbf{NOC}}                       & \multicolumn{2}{c}{\textbf{IFANIN}}                           \\
                       & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before}       & \multicolumn{1}{c}{after}        & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} &  \\
\midrule
\textbf{Upper whisker}
& 85.00                      & 38.59                     & 2.62                       & 3.00                      & 16.33                      & 18.10                     & 4.44                       & 4.89                      & 6.26                       & 6.56                      & 2.50                       & 2.50                      & 21.43                      & 22.26                     & 19.50                      & 22.00                     & 93.00                      & 93.00                     & 2.22                             & 1.89                             & 16.08                      & 10.76                     & 1.92                       & 1.82                      & 2.62                       & 3.00                      & 0.82                       & 0.79                      & 1.69                       & 1.71                      \\ 
\textbf{3rd Q}         & 48.93                      & 37.61                     & 1.65                       & 1.60                      & 9.44                       & 9.43                      & 3.17                       & 3.25                      & 4.64                       & 4.53                      & 1.54                       & 1.51                      & 12.47                      & 12.76                     & 11.33                      & 12.00                     & 51.44                      & 54.08                     & 1.50                             & 1.38                      & 8.83                       & 6.67                      & 1.10                       & 1.09                      & 1.59                       & 1.60                      & 0.33                       & 0.35                      & 1.29                       & 1.29                      \\
\textbf{Median}        & 28.12                      & 25.86                     & 1.09                       & 1.00                      & 5.94                       & 5.91                      & 2.75                       & 2.70                      & 3.67                       & 3.71                      & 1.20                       & 1.14                      & 7.43                       & 7.26                      & 7.00                       & 7.75                      & 32.49                      & 34.31                     & 1.13                             & 1.12                             & 2.84                       & 2.42                      & 0.71                       & 0.67                      & 1.09                       & 1.00                      & 0.15                       & 0.19                      & 1.13                       & 1.14                   \\
\textbf{1st Q}         & 23.34                      & 17.69                     & 0.71                       & 0.60                      & 3.82                       & 3.58                      & 2.16                       & 2.05                      & 3.06                       & 3.01                      & 0.88                       & 0.84                      & 5.05                       & 5.33                      & 5.00                       & 5.00                      & 16.30                      & 20.78                     & 1.01                             & 1.02                             & 1.81                       & 1.67                      & 0.52                       & 0.50                      & 0.71                       & 0.63                      & 0.00                       & 0.04                      & 1.00                       & 1.00                      \\
\textbf{Lower whisker} & 14.38                      & 8.45                      & 0.00                       & 0.00                      & 0.84                       & 0.92                      & 1.00                       & 0.89                      & 1.62                       & 1.22                      & 0.00                       & 0.00                      & 0.75                       & 1.12                      & 1.47                       & 1.92                      & 0.00                       & 0.00                      & 0.67                             & 0.75                             & 0.00                       & 0.00                      & 0.00                       & 0.00                      & 0.00                      & 0.00                      & 0.00                       & 0.00                      & 0.71                       & 0.78                      \\
\textbf{Mean}          & 38.86                      & 32.99                     & 1.21                       & 1.10                      & 7.79                       & 7.88                      & 2.78                       & 2.71                      & 3.81                       & 3.78                      & 1.42                       & 1.33                      & 9.55                       & 9.81                      & 10.15                      & 10.70                     & 35.98                      & 37.55                     & 1.40                             & 1.32                             & 42.29                      & 27.83                     & 0.84                       & 0.80                      & 1.20                       & 1.11                      & 0.22                       & 0.24                      & 1.19                       & 1.19   \\ 


\midrule 
\multirow{3}{*}{}      &
\multicolumn{12}{c}{\textbf{Design Size}}                                                                                                 & \multicolumn{4}{c}{\textbf{Encapsulation}}                                                                      & \multicolumn{4}{c}{\textbf{Abstraction}}                                                                        & \multicolumn{4}{c}{\textbf{Polymorphism}}                                                                                                                                        \\
                    \cmidrule{2-26}
                    & \multicolumn{2}{c}{\textbf{LOC}}                       & \multicolumn{2}{c}{\textbf{CLOC}}                      & \multicolumn{2}{c}{\textbf{STMTC}}                     & \multicolumn{2}{c}{\textbf{CDL}}                       & \multicolumn{2}{c}{\textbf{NIV}}                       & \multicolumn{2}{c}{\textbf{NIM}}                       & \multicolumn{2}{c}{\textbf{WMC}}                       & \multicolumn{2}{c}{\textbf{LCOM}}                      & \multicolumn{2}{c}{\textbf{WMC}}                       & \multicolumn{2}{c}{\textbf{LCOM}}                      & \multicolumn{2}{c}{\textbf{WMC}}                       & \multicolumn{2}{c}{\textbf{RFC}}  
                                                \\
                       & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before}       & \multicolumn{1}{c}{after}        & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} & \multicolumn{1}{c}{before} & \multicolumn{1}{c}{after} &   \\
\midrule
\textbf{Upper whisker}
& 95.70                      & 97.43                     & 20.86                      & 22.80                     & 42.96                      & 42.96                     & 3.12                       & 3.50                      & 12.33                      & 11.00                     & 12.33                      & 11.00                     & 20.80                      & 20.62                     & 55.11                      & 70.50                     & 19.90                      & 18.44                     & 68.17                      & 66.75                     & 17.40                      & 17.10                     & 18.44                      & 16.38                     \\
\textbf{3rd Q}                               & 64.44                      & 63.08                     & 11.92                      & 12.51                     & 31.38                      & 30.76                     & 2.67                       & 2.88                      & 6.07                       & 5.88                      & 6.07                       & 5.88                      & 11.79                      & 11.69                     & 42.00                      & 44.42                     & 11.08                      & 10.70                     & 39.07                      & 38.78                     & 11.12                      & 11.47                     & 11.55                      & 13.50                     \\
\textbf{Median}                              & 49.29                      & 49.60                     & 7.97                       & 7.55                      & 23.57                      & 24.22                     & 1.82                       & 1.66                      & 4.00                       & 3.76                      & 4.00                       & 3.76                      & 8.28                       & 8.19                      & 34.18                      & 32.50                     & 7.26                       & 7.00                      & 26.57                      & 24.81                     & 9.38                       & 9.70                      & 6.00                       & 6.50                      \\
\textbf{1st Q } & 40.20                      & 40.02                     & 5.62                       & 5.53                      & 19.63                      & 20.03                     & 0.91                       & 1.00                      & 1.40                       & 1.67                      & 1.40                       & 1.67                      & 5.33                       & 5.67                      & 25.95                      & 25.91                     & 5.11                       & 5.24                      & 16.39                      & 16.67                     & 5.00                       & 5.05                      & 4.00                       & 4.22                      \\
\textbf{Lower whisker} & 27.40                      & 30.21                     & 0.42                       & 1.13                      & 11.55                      & 11.52                     & 0.33                       & 0.33                      & 0.27                       & 0.50                      & 0.27                       & 0.50                      & 2.79                       & 3.16                      & 2.39                       & 2.16                      & 0.60                       & 0.60                      & 0.00                       & 0.00                      & 1.50                       & 1.58                      & 2.50                       & 1.25                      \\
\textbf{Mean} & 58.14                      & 57.30                     & 11.24                      & 11.14                     & 29.34                      & 28.81                     & 3.29                       & 3.21                      & 4.81                       & 4.76                      & 4.81                       & 4.76                      & 9.42                       & 9.58                      & 38.28                      & 37.78                     & 9.55                       & 8.92                      & 29.52                      & 28.67                     & 8.92                       & 9.19                      & 10.46                      & 10.38                    
\\

     \bottomrule
\end{tabular} 
\end{adjustbox}
%\end{sideways}
\end{center}
\end{table*}







==> Tables/QualityImpactSummary.tex <==
\begin{table*}[!htbp]
\begin{center}
\caption{Overall Impact of SAR on Quality - Summary}
\label{Table:Impact of SAR on Quality}
\begin{adjustbox}{width=0.8\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lcccccccc}

\toprule
\multirow{2}{*}{\textbf{Software Metrics}} & \multicolumn{8}{c}{\textbf{Quality Attribute}}                                                            \\
\cmidrule{2-9}
                                           & Cohesion & Coupling & Complexity & Inheritance & Polymorphism & Encapsulation & Abstraction & Design Size \\
\midrule                                           
LCOM                                       & +ve      &          & -ve        &             &              & +ve           & +ve         &             \\
CBO                                        &          & +ve      &            &             &              &               &             &             \\
RFC                                        &          & +ve      & -ve        &             & -ve          &               &             &             \\
FANIN                                      &          & +ve      &            &             &              &               &             &             \\
FANOUT                                     &          & -ve      &            &             &              &               &             &             \\
CC                                         &          &          & +ve        &             &              &               &             &             \\
WMC                                        &          &          & +ve        &             & -ve          & +ve           & +ve         &             \\
Evg                                        &          &          & +ve        &             &              &               &             &             \\
NPATH                                      &          &          & +ve        &             &              &               &             &             \\
MaxNest                                    &          &          & +ve        &             &              &               &             &             \\
DIT                                        &          &          &            & +ve         &              &               &             &             \\
NOC                                        &          &          &            & -ve         &              &               &             &             \\
IFANIN                                     &          &          &            & -ve         &              &               &             &             \\
LOC                                        &          &          &            &             &              &               &             & -ve         \\
CLOC                                       &          &          &            &             &              &               &             & +ve         \\
STMTC                                      &          &          &            &             &              &               &             & -ve         \\
CDL                                        &          &          &            &             &              &               &             & +ve         \\
NIV                                        &          &          &            &             &              &               &             & +ve         \\
NIM                                        &          &          &            &             &              &               &             & +ve \\     
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}
